Environment Classification via Blind Roomprints Estimation

In this paper we present a novel approach for environment classification for speech recordings, which does not require the selection of decaying reverberation tails. It is based on a multi-band RT60 analysis of blind channel estimates and achieves an accuracy of up to 93.6% on test recordings derived from the ACE corpus.

==> _useful_notes.tex <==
\cleardoublepage

\section{Skeleton}

\begin{enumerate}
    \item Introduction
    \begin{itemize}
        \item Environment classification (part of audio forensics) aims at determining where a recording took place~\cite{Roomprints:AES:2014,Roomprints:IEEE:2013}
        \item Could help immensely in both fight against disinformation and in court cases, by identifying disagreements between the recording characteristics and the allegations
        \item Is challenging -- the existing literature struggle to reach an accuracy which can be used in real-life speech content~\cite{EnvClass:Patole:CAST,EnvClass:Malik:ICASSP}. 
        \item In this paper we propose to address the problem by multi-band RT60 analysis of blind channel estimates. Multi-band RT60 analysis has been proposed as essential component for deriving roomprint features for environment classification in~\cite{Roomprints:AES:2014,Roomprints:IEEE:2013}. In the original reference works, these features were retrieved in laboratory conditions, by analysing the noiseless room impulse response in the time domain. Our proposal is instead relying on a blind estimate of the existing transmission channel~\cite{Gaubitch:ChannelEstimation}, which is used as source for estimating the desired roomprints. Notably, our proposed approach is applicable on speech recordings without the need for (semi-)automatic selection of decaying reverberation tails, which is prone to error and might lead to increased error rates.
        \item The rest of the paper is organized as follows
    \end{itemize}
    \item Background
    \begin{itemize}
        \item Roomprints for environment classification definition as in \cite{Roomprints:AES:2014,Roomprints:IEEE:2013}
        \item Limitations due to the laboratory environment
        \item Connection between RIR $h(t)$ and estimated $\hat h(t)$ to overcome the limitation
    \end{itemize}
    \item Proposed Approach
    \begin{enumerate}
        \item Blind Channel Magnitude Estimation
        \begin{itemize}
            \item Model of $x = h * s$
            \item Statistical modeling of clean speech
            \item Blind channel estimation
        \end{itemize}
        \item Blind Minimal-Phase Channel Estimation
        \begin{itemize}
            \item (?)Griffin-Lim Algorithm
            \item Invfreqz-based approach
        \end{itemize}
        \item Blind Roomprint Estimation
        \begin{itemize}
            \item Retrieve $\hat h(t)$
            \item Fractional-octave band filtering
            \item Feature vector creation 
        \end{itemize}
        \item Classification Algorithm
    \end{enumerate}
    \item Evaluation
    \begin{enumerate}
        \item Dataset Description
        \item Evaluation Metrics
        \item Experimental Setup
        \item Results
    \end{enumerate}
    \item Conclusions and Outlook
        \begin{itemize}
        \item TODO: influence of noise via AI / Gaubitch 
        \item TODO: influence of microphone device
    \end{itemize}
\end{enumerate}

\vfill\null
\section{Useful Notes}

\begin{itemize}
    \item Full-paper: max 6 pages \emph{including} references
    \item Biblatex is used as backend: type \citeauthor{Cuccovillo:2016:ICASSP}~\cite{Cuccovillo:2016:ICASSP} instead of Cuccovillo et al.~\cite{Cuccovillo:2016:ICASSP}
    \item Cleveref is loaded: type \Cref{fig:fancy-unicorn} instead of Figure~\ref{fig:fancy-unicorn} if you need a cross-reference
\end{itemize}

\begin{figure}[hb]
  \centering
  \includegraphics[width=\linewidth]{img/fancy-unicorn}
  \caption{Lucky-charm for a successful submission}\label{fig:fancy-unicorn}
\end{figure}

==> img/filter-bandwidth-comparison.tex <==
\begin{figure*}[t]
  \begin{minipage}[b]{\confmatminipagewidth}
    \centering
    \includegraphics[width=\confmatwidth]{img/fancy-unicorn}
    \subcaption{$1/3$-octave}
  \end{minipage}%
  \begin{minipage}[b]{\confmatminipagewidth}
    \centering
    \includegraphics[width=\confmatwidth]{img/fancy-unicorn}
    \subcaption{$1/4$-octave}
  \end{minipage}%
  \begin{minipage}[b]{\confmatminipagewidth}
    \centering
    \includegraphics[width=\confmatwidth]{img/fancy-unicorn}
    \subcaption{$1/8$-octave}
  \end{minipage}
   \caption{Outcome of environment classification for varying fractional-octave filter bandwidths}\label{fig:eval:filter-bandwidth}
\end{figure*}
